Bayesian Nash Equilibrium in First-Price Auction with Discrete Value Distributions

First price auctions are widely used in government contracts and industrial auctions. In this paper, we consider the Bayesian Nash Equilibrium (BNE) in first price auctions with discrete value distributions. We study the characterization of the BNE in the first price auction and provide an algorithm to compute the BNE at the same time. Moreover, we prove the existence and the uniqueness of the BNE. Some of the previous results in the case of continuous value distributions do not apply to the case of discrete value distributions. In the meanwhile, the uniqueness result in discrete case cannot be implied by the uniqueness property in the continuous case. Unlike in the continuous case, we do not need to solve ordinary differential equations and thus do not suffer from the solution errors therein. Compared to the method of using continuous distributions to approximate discrete ones, our experiments show that our algorithm is both faster and more accurate. The results in this paper are derived in the asymmetric independent private values model, which assumes that the buyers' value distributions are common knowledge.

==> 3_reserve.tex <==
\section{First price auctions with reserve prices}
%Players who bid larger than or equal to their reserves enter the first price auction. In previous sections, we do not consider reserves or we can think in the way that reserves are zeros.
%In this section, we show the result can be easily generalized to the homogeneous reserves. While for the heterogeneous reserves, new difficulty emerges. This new difficulty comes from players' atom bid on their reserves.

\subsection{homogeneous reserve prices}
%When players have homogeneous reserve $r$, the smallest winning bid might need modification. Assume $\underline{b}$ is calculated in Lemma~\ref{lemma3}, i.e., the smallest winning bid with no reserves. We first consider the easy case $r\leq \underline{b}$. In this case, BNE remains the same since all winning bids are larger than $r$.
%
%If $r>\underline{b}$, players who bid $\underline{b}$ cannot enter the auction. The new smallest winning bid $\underline{b}^*$ will be at least $r$.
%In fact  $\underline{b}^*$ equals $r$ otherwise the player who bids  $\underline{b}^*$ has an incentive to deviate to  bid $r$.
%To accommodate the change, we claim our algorithm 2 finds the correct BNE when the smallest winning bid matches $r$.

We can reduce the problem to the case with no reserve by decreasing every players' values. Given value distribution G and reserve r, we define new  distribution $G^*(x)=G(x+r),~x\geq 0$. Then we compute $s^*_i(x)~\forall i$ in BNE for $G^*$ with no reserve.
The strategy in equilibrium also decrease by $r$. Therefore we can reconstruct the BNE by strategy $s_i(x)=s^*_i(x)+r$ if $x\geq r$ and $s(x)=0 $ if $x< r$.

\subsection{heterogeneous reserve prices}
We give an example with three players. Player 1's value is 12. Players 2 and 3 have two different types. They have three different reserves $r_1=0$, $r_2=1$ and $r_3=7$. The distribution is given in Example \ref{eg_3_reserve}. 
\begin{example}
    \label{eg_3_reserve}
    \[
    G_1(12)=1 \quad
    G_2(x)=\begin{cases}
    1,& x=14\\
    \frac{\sqrt{6}}{6},& x=0.5\\
    \end{cases}\quad
    G_3(x)=\begin{cases}
    1,& x=12\\
    \frac{\sqrt{6}}{6},& x=6\\
    \end{cases}  
    \]
    The bid distribution in BNE is the following.
    \[
    F_1(x)=\begin{cases}
    2(14-x)^{-1/2},& x\in[8,10]\\
    4\sqrt{6}(14-x)^{-1},  & x\in[1,2]\\
    \frac{\sqrt{6}}{3}, & x=0 \\
    \end{cases}
    \quad
    F_2(x)=\begin{cases}
    (12-x)^{-1}(14-x)^{1/2},& x\in(8,10]\\
    \sqrt{6}(12-x)^{-1},& x\in(7,8]\\
    2\sqrt{6}(12-x)^{-1},& x\in[1,2]\\
    \end{cases}
    \]
    \[            
    F_3(x)=\begin{cases}
    2(14-x)^{-1/2},& x\in(8,10]\\
    2\sqrt{6}(14-x)^{-1}, & x\in[7,8]\\
    \end{cases}  
    \]
\end{example}

\begin{figure}[h]
	\centering
\includegraphics[width=0.45\linewidth]{figures/3_reserve}
	\caption{A dot means there is a positive probability. They all have atom bid at their reserve prices. No buyer gives a bid in $(2,7)$. Buyer 1 leaves the bidding set at bid $8$}
\end{figure}
In this example, buyer 3 has an atom bid on his reserve $r_3$.
Because the existence of the atom bid above the smallest winning bid,
Theorem \ref{thmbidcont} does not hold anymore. Even if we consider continuous value distributions, this gaps still exist.
No buyer bids in lower neighbor interval around it otherwise he has an incentive to bid $r_3+\epsilon$ which gives him a large increase of winning probability, but only sacrifices a little in the utility conditioned on winning.

Both buyer 1 and buyer 2 have gaps in their bid supports, $(2,8)$ and $(2,7)$. It can be shown that these two gaps always share the same lower endpoints. But the higher endpoints are different, e.g., buyer 1 leaves the bidding set at 8 while buyer 2 leaves the bidding set at 7.
Until now, we do not have an easy method to compute the positions of these gaps directly, and similar to the backward-shooting algorithm, we may need to guess all these gaps.
In summary, to compute BNE with heterogeneous reserve prices, we have to guess not only the largest winning bid but also the positions of all gaps in the bid support.














